Traversing Between Modes in Function Space for Fast Ensembling

Deep ensemble is a simple yet powerful way to improve the performance of deep neural networks. Under this motivation, recent works on mode connectivity have shown that parameters of ensembles are connected by low-loss subspaces, and one can efficiently collect ensemble parameters in those subspaces. While this provides a way to efficiently train ensembles, for inference, multiple forward passes should still be executed using all the ensemble parameters, which often becomes a serious bottleneck for real-world deployment. In this work, we propose a novel framework to reduce such costs. Given a low-loss subspace connecting two modes of a neural network, we build an additional neural network that predicts the output of the original neural network evaluated at a certain point in the low-loss subspace. The additional neural network, which we call a "bridge", is a lightweight network that takes minimal features from the original network and predicts outputs for the low-loss subspace without forward passes through the original network. We empirically demonstrate that we can indeed train such bridge networks and significantly reduce inference costs with the help of bridge networks.

==> main/misc.tex <==

\section*{Accessibility}
Authors are kindly asked to make their submissions as accessible as possible for everyone including people with disabilities and sensory or neurological differences.
Tips of how to achieve this and what to pay attention to will be provided on the conference website \url{http://icml.cc/}.

\section*{Software and Data}

If a paper is accepted, we strongly encourage the publication of software and data with the
camera-ready version of the paper whenever appropriate. This can be
done by including a URL in the camera-ready copy. However, \textbf{do not}
include URLs that reveal your institution or identity in your
submission for review. Instead, provide an anonymous URL or upload
the material as ``Supplementary Material'' into the CMT reviewing
system. Note that reviewers are not required to look at this material
when writing their review.

% % Acknowledgements should only appear in the accepted version.
% \section*{Acknowledgements}

% \textbf{Do not} include acknowledgements in the initial version of
% the paper submitted for blind review.

% If a paper is accepted, the final camera-ready version can (and
% probably should) include acknowledgements. In this case, please
% place such acknowledgements in an unnumbered section at the
% end of the paper. Typically, this will include thanks to reviewers
% who gave useful comments, to colleagues who contributed to the ideas,
% and to funding agencies and corporate sponsors that provided financial
% support.


==> table/distill.tex <==
\begin{table*}[t]
    \caption{FLOPs, $R^2$ scores, and model performance metrics between type I bridge network and \gls{cnn}$^\text{(ft)}$ $\times n$ $+$ \gls{cnn} models with various sizes on CIFAR-100. Here, $\times n$ denotes the number of convolution layers to use as a frontal feature extractor \gls{cnn}$^\text{(ft)}$, and \gls{cnn} denotes the same architecture used in the type I bridge network. $R^2$ scores are measured with respect to the target Bezier $r=0.5$.}
    \centering
    \vskip 0.05in
    \def\arraystretch{1.1}
    \resizebox{0.95\columnwidth}{!}{
        \begin{tabular}{lrllllll}
            \toprule
            Model                                         & FLOPs ($\downarrow$) & $R^2$ ($\uparrow$)          & ACC ($\uparrow$)           & NLL ($\downarrow$)          & ECE ($\downarrow$)          & BS ($\downarrow$)           \\
            \midrule
            Type I Bridge                                 & $\times$ 0.211       & \textBF{0.786} $\pm{0.003}$ & \textBF{72.18} $\pm{0.19}$ & \textBF{1.016} $\pm{0.004}$ &         0.031  $\pm{0.002}$ & \textBF{0.379} $\pm{0.001}$ \\
            \cmidrule(lr){1-7}
            \gls{cnn}$^\text{(ft)}$ $\times$2 $+$ \gls{cnn} & $\times$ 0.230       &         0.626  $\pm{0.007}$ &         63.45  $\pm{0.71}$ &         1.318  $\pm{0.019}$ &         0.015  $\pm{0.002}$ &         0.481  $\pm{0.007}$ \\
            \gls{cnn}$^\text{(ft)}$ $\times$4 $+$ \gls{cnn} & $\times$ 0.373       &         0.682  $\pm{0.005}$ &         67.39  $\pm{0.42}$ &         1.166  $\pm{0.015}$ &         0.013  $\pm{0.001}$ &         0.436  $\pm{0.004}$ \\
            \gls{cnn}$^\text{(ft)}$ $\times$6 $+$ \gls{cnn} & $\times$ 0.515       &         0.685  $\pm{0.006}$ &         67.43  $\pm{0.55}$ &         1.156  $\pm{0.019}$ &         0.014  $\pm{0.001}$ &         0.433  $\pm{0.006}$ \\
            \gls{cnn}$^\text{(ft)}$ $\times$8 $+$ \gls{cnn} & $\times$ 0.648       &         0.701  $\pm{0.001}$ &         68.36  $\pm{0.35}$ &         1.121  $\pm{0.009}$ & \textBF{0.012} $\pm{0.002}$ &         0.422  $\pm{0.004}$ \\
            \bottomrule
        \end{tabular}
    }
    \label{tab:distill}
\end{table*}

==> table/type1_increase.tex <==
\begin{table*}[t]
    \color{red}
    \caption{\color{red}Performance gain of a single ResNet model with respect to the $n$ type I bridge networks where $n$ denotes the number of additional type I bridge networks on CIFAR-100 dataset.} 
    \centering
    \vskip 0.07in
    \resizebox{0.6\textwidth}{!}{
        \begin{tabular}{lrlll}
            \toprule
            Model             & FLOPs ($\downarrow$) & ACC ($\uparrow$)           & NLL ($\downarrow$)          & DEE ($\uparrow$)            \\
            \midrule
            ResNet            & $\times$ 1.000       &         72.79  $\pm{0.44}$ &         1.107  $\pm{0.005}$ &         1.000               \\
            \quad + 1 Bridge  & $\times$ 1.017       &         73.14  $\pm{0.27}$ &         1.069  $\pm{0.003}$ &         1.256  $\pm{0.046}$ \\
            \quad + 2 Bridges & $\times$ 1.034       &         73.23  $\pm{0.29}$ &         1.056  $\pm{0.004}$ &         1.346  $\pm{0.055}$ \\
            \quad + 4 Bridges & $\times$ 1.067       &         73.33  $\pm{0.34}$ &         1.047  $\pm{0.004}$ &         1.403  $\pm{0.051}$ \\
            \quad + 6 Bridges & $\times$ 1.101       & \textBF{73.41} $\pm{0.33}$ & \textBF{1.044} $\pm{0.004}$ & \textBF{1.426} $\pm{0.053}$ \\
            \bottomrule
        \end{tabular}
    }
    \label{tab:number_of_type_1_and_performance}
\end{table*}

